Scalable Bayesian Inference for Detection and Deblending in Astronomical Images

We present a new probabilistic method for detecting, deblending, and cataloging astronomical sources called the Bayesian Light Source Separator (BLISS). BLISS is based on deep generative models, which embed neural networks within a Bayesian model. For posterior inference, BLISS uses a new form of variational inference known as Forward Amortized Variational Inference. The BLISS inference routine is fast, requiring a single forward pass of the encoder networks on a GPU once the encoder networks are trained. BLISS can perform fully Bayesian inference on megapixel images in seconds, and produces highly accurate catalogs. BLISS is highly extensible, and has the potential to directly answer downstream scientific questions in addition to producing probabilistic catalogs.

==> former_introduction.tex <==
\section{Introduction}
% \begin{itemize}
%   \item What is detecting?
%   \item What is a blend, and what is deblending?
%   \item What does the data look like? Why is scalability important?
          %   \end{itemize}
Astronomical images are the primary way in which we learn about the universe.
Given an astronomical image, our goal is to uncover the catalog of objects that make up an area of the night sky. \ismael{Might be good to mention briefly one or two applications of accurate astronomical catalogs (I can add it)} \ismael{Might 'best possible estimate given this image of the catalog of objects...' be better than 'uncover'? We can never uncover this catalog as our instruments are not perfect.}
Astronomical catalogs consist of the type, location, apparent brightness (flux), color, and morphology of each object.

To find these objects, astronomers have historically used software pipelines based on fixed rules.
For example, one procedure identifies an object as a bright pixel surrounded by a $7 \times 7$ grid of dimmer pixels \citep{anderson2016empirical}.
These algorithms give reasonable results when the pixels corresponding to each object are well separated from each other in a given image. However, they struggle with handling ambiguity in regions where multiple objects are overlap with each other, an effect known as \textit{blending}.
\ismael{There are other algorithms (like scarlet) that go beyond explicit rules like this one, I wonder if we should mention them}

For example, an apparent bright object could be one bright object or multiple dimmer objects blended together. 
These algorithms also require developing explicit rules, a challenging and time-consuming task.

In contrast, our probabilistic approach directly models how stars and galaxies are distributed in the night sky and how these objects lead to the observed image.
Specifically, we choose a prior distribution over all possible catalogs in a region of the sky.
Then, conditioned on a particular catalog, the number of photoelectrons in each pixel follows a Poisson distribution whose rate corresponds to the number and brightness of nearby objects. \ismael{should we say explicitly the last sentence is the likelihood? or is it obvious enough?} 

With the prior and likelihood specified, our goal is to infer the posterior distribution of the catalog conditional on the observed image.
When objects are bright and isolated, point estimates from a probabilistic approach will match heuristic approaches. \ismael{is it clear that 'heuristic approaches' means 'rule based' or 'classical' approaches?}
However, performing inference through a posterior distribution has two key advantages.
First, explicit rules are no longer needed.
The event of an object being placed at a particular location is based on the combined information from the prior and the likelihood.
For example, apparent bright spots will result in a detection based on the relative probabilities of inclusion and exclusion, not an arbitrary rule.
Working with probabilities is particularly advantageous for the task of \textit{deblending}, or separating two or more light sources that overlap in an image.
With a heuristic approach, special rules need to be put in place to detect blends \revise{(cite)}. \ismael{Again, there are algorithms with more principled deblending approaches. But I think I remember SExtractor being rule based, so we could cite that...}
However, deblending is naturally achieved in a probabilistic framework with no need for special rules.
Detecting blends is a matter of evaluating whether the probability of a bright spot is higher as multiple overlapping objects or a singular object.

This leads to the second key advantage of a probabilistic approach: the ability to quantify the ambiguity in astronomical images.
In crowded areas where light sources are blended together, the posterior distribution of the catalog will correctly reflect the uncertainty in the number of light sources, their locations, and their fluxes.
Quantifying this uncertainty in the posterior distribution of catalogs allows for these ambiguities to be handled better in downstream tasks.

Our proposed model, the Bayesian Light Source Separator (BLISS), enables the benefits of probabilistic cataloging while maintaining the capability to scale to entire astronomical surveys.
Rather than use MCMC to draw samples, BLISS utilizes \textit{variational inference} (VI).
With VI, we optimize the parameters of a tractable family of distributions that is close to the posterior in terms of Kullback Lielber (KL) divergence.
While traditional VI approaches lead to a significant speed up over MCMC \citep{regier2019approximate}, they still require optimizing parameters for each new portion of the sky, which is costly.
To avoid retraining with each new image, BLISS leverages \textit{amortized} VI \revise{(cite)}, where an encoder neural network takes in an image and outputs the variational parameters.
After a training period of a few hours, BLISS can catalog an unseen 1500x2000 SDSS frame in just 10 seconds on a single GPU.
Moreover, since training is fixed cost and only performed once, BLISS has the potential to scale up to entire astronomical surveys with ease.

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{./figures/drawings/generative_model.png}
  \caption{
    BLISS Generative model
  }\label{fig:generative}
\end{figure}

% BLISS builds on two previous variational inference approaches to cataloging.
% Each of these approaches have significant limitations, which BLISS is able to overcome.
% \cite{regier2019approximate} used variational inference to catalog stars and galaxies. However, the authors relied on deterministic preprocessing routines for detection, making it unsuitable for crowded fields; in crowded fields detections are a major source of uncertainty. Furthermore, \cite{regier2019approximate} used a simplistic galaxy model, which the authors identified as a significant source of model misspecification.
% \cite{liu2021variational} used stochastic variational inference to deblend crowd starfields. We follow their general approach, but extend it deblend galaxies too. Our work is a major extension because galaxies are much more complex than stars. Whereas stars are well modeled as point sources, such that nearby stars differ only by apparent brightness, galaxies have spatial extent; their appearances are not well described by any simple parametric model.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/decals_accuracy.tex <==
17 - 18 & 0.96 & 1.00 & 0.95& 0.96 & 1.00 & 0.94 \\
18 - 19 & 1.00 & 1.00 & 1.00& 1.00 & 1.00 & 1.00 \\
19 - 20 & 0.99 & 1.00 & 0.96& 1.00 & 1.00 & 1.00 \\
20 - 21 & 0.91 & 0.89 & 0.96& 0.90 & 0.85 & 0.98 \\
21 - 22 & 0.77 & 0.84 & 0.64& 0.82 & 0.79 & 0.89 \\
22 - 23 & 0.58 & 0.62 & 0.51& 0.60 & 0.60 & 0.60 \\
Overall & 0.83 & 0.84 & 0.81& 0.84 & 0.81 & 0.88 \\


==> tables/decals_detections.tex <==
17 - 18 & 28 & 27 & 2 & 23 & 2 \\
18 - 19 & 44 & 40 & 3 & 38 & 4 \\
19 - 20 & 80 & 70 & 7 & 65 & 7 \\
20 - 21 & 150 & 136 & 8 & 127 & 7 \\
21 - 22 & 290 & 211 & 29 & 210 & 31 \\
22 - 23 & 520 & 105 & 75 & 100 & 36 \\
Overall & 1139 & 612 & 132 & 586 & 94 \\

